Improving Zero and Few-Shot Abstractive Summarization with Intermediate Fine-tuning and Data Augmentation

Models pretrained with self-supervised objectives on large text corpora achieve state-of-the-art performance on English text summarization tasks. However, these models are typically fine-tuned on hundreds of thousands of data points, an infeasible requirement when applying summarization to new, niche domains. In this work, we introduce a novel and generalizable method, called WikiTransfer, for fine-tuning pretrained models for summarization in an unsupervised, dataset-specific manner. WikiTransfer fine-tunes pretrained models on pseudo-summaries, produced from generic Wikipedia data, which contain characteristics of the target dataset, such as the length and level of abstraction of the desired summaries. WikiTransfer models achieve state-of-the-art, zero-shot abstractive summarization performance on the CNN-DailyMail dataset and demonstrate the effectiveness of our approach on three additional diverse datasets. These models are more robust to noisy data and also achieve better or comparable few-shot performance using 10 and 100 training examples when compared to few-shot transfer from other summarization datasets. To further boost performance, we employ data augmentation via round-trip translation as well as introduce a regularization term for improved few-shot transfer. To understand the role of dataset aspects in transfer performance and the quality of the resulting output summaries, we further study the effect of the components of our unsupervised fine-tuning data and analyze few-shot performance using both automatic and human evaluation.

==> helpers_old.tex <==

% SECTION: zero-shot tables
\newcommand{\ZeroShotAllDatasets}{
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{c | c c c | c c c c } \Xhline{2\arrayrulewidth}
             \textbf{Target Dataset} &  \multicolumn{3}{c|}{\textbf{WikiTransfer}} & \multicolumn{4}{c}{\textbf{Other Transfer}}   \\ \Xhline{\arrayrulewidth}
              CNNDM & \textbf{39.11} & \textbf{17.25} & \textbf{35.73} & 36.81 & 14.18 & 32.62 &  (Reddit)   \\
              XSum & \textbf{31.85} & \textbf{10.44} & \textbf{23.75} & 24.04 & 6.43 & 18.99 &  (Reddit)   \\ 
             Reddit & \textbf{21.47} & 4.10 & 17.62 & 21.37 & \textbf{4.14} & \textbf{17.76} &  (CNNDM)  \\
             BigPatent & \textbf{35.58} & \textbf{10.91} & \textbf{31.53} & 33.57 & 9.34 & 25.76 & (CNNDM)    \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Comparison of ROUGE-1/2/L zero-shot transfer performance from dataset-specific WikiTransfer vs. transfer from another dataset. The dataset from which zero-shot transfer performed the best is in parentheses.}
\label{tab:zero_shot}
\end{table}
}

\newcommand{\UnsupComparison}{
\begin{table}[t!]
\tiny
\centering
\resizebox{.8\columnwidth}{!}{\begin{tabular}{c c c c} \Xhline{2\arrayrulewidth}
             \textbf{Model} & \multicolumn{3}{c}{\textbf{ROUGE-1/2/L}}   \\
              WikiTransfer & \textbf{39.11} & \textbf{17.25} & \textbf{35.73} \\
              TED \cite{yang-etal-2020-ted}  & 38.73 & 16.84 & 35.40  \\
             \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{A comparison of our approach to the unsupervised pretraining of TED \cite{yang-etal-2020-ted}, showing the superior performance and generalizability of our approach versus the TED model, which focused specifically on the news domain.}
\label{tab:unsup_comparison}
\end{table}
}

% SECTION: zero-shot ablation studies
\newcommand{\SentenceChoiceComparison}{
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{c c c c} \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} & \textbf{First M Sents} & \textbf{IND-ORIG} & \textbf{IND-ORIG-P}   \\  \Xhline{2\arrayrulewidth}
             CNNDM &  40.14/17.71/36.66  & 37.62/15.15/34.21   &  37.85/15.32/34.39 \\
             XSum & 31.80/10.46/23.66 & 29.95/9.37/21.78  & 30.22/9.79/23.23 \\
             \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{A comparison of the effect of summary sentence choice for WikiTransfer on zero-shot transfer ROUGE-1/2/L performance.}
% \lhr{same problem as previous table}
\label{tab:sentence_choice_comparison}
\end{table}
}
\newcommand{\DatasetSizeComparison}{
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{c | c c c | c c c  } \Xhline{2\arrayrulewidth}
            \textbf{Intermediate Dataset Size} &  \multicolumn{3}{c}{\textbf{CNNDM}} &  \multicolumn{3}{c}{\textbf{XSum}}  \\  \Xhline{2\arrayrulewidth}
              10k & 39.48 & 17.79 & 36.3 & 21.59 & 4.85 & 16.28 \\
              100k & 39.92 & 17.65 & 36.5 & 31.52 & 10.86 & 23.94 \\
              250k & 40.10 & 17.70 & 36.62 & 31.39 & 10.27 & 23.43 \\
              400k & 40.14 & 17.71 & 36.66 & 31.80 & 10.46 & 23.66 \\
             \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{A comparison of the effect of dataset size of the unsupervised intermediate fine-tuning data on the zero-shot transfer ROUGE-1/2/L performance.} 
\label{tab:dataset_size_comparison}
\end{table}
}


\newcommand{\AblationsLRBinM}{
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{c | c c c | c c c } \Xhline{2\arrayrulewidth}
            \textbf{Ablation} & \multicolumn{3}{c}{ \textbf{CNNDM}} & \multicolumn{3}{c}{\textbf{XSum}}  \\ \hline
              LR=3e-6 & 40.14 & 17.71 & 36.66 & 27.60 & 8.62 & 20.93 \\
              LR=3e-5 & 39.73 & 16.94 & 36.24 & 31.80 & 10.46 & 23.66 \\ \hline
              LR=3e-6, No-bin & 39.11 & 16.98 & 35.66 & 22.78 & 5.66 & 17.16  \\ \hline
              LR=3e-6, bin, M=1 & 37.45 & 14.72 & 32.52 & 27.60 & 8.62 & 20.93   \\ 
              LR=3e-6, bin, M=3  &  40.14 & 17.71 & 36.66 & 27.98 & 9.59 & 23.11  \\ \hline
             \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Ablation studies on the effect of learning rate, the use of extractive bin for data filtering and the choice of M in intermediate fine-tuning on ROUGE-1/2/L performance on CNNDM and XSum validation sets. 
}
\label{tab:ablations_lr_bin_m}
\end{table}
}


\newcommand{\TableAll}{
\begin{table}[t!]
\tiny
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{ c c c c } \Xhline{2\arrayrulewidth}
            % CNNDM
             \textbf{Target Dataset} &  \multicolumn{3}{c}{CNNDM}  \\
             \Xhline{2\arrayrulewidth}
             \textbf{Transfer from} & WikiTransfer & Reddit & BART \\ \Xhline{2\arrayrulewidth}
            \textbf{0} & \textbf{39.11/17.25/35.73} & 36.81/14.18/32.62 & 35.98/15.10/32.97  \\  \Xhline{2\arrayrulewidth}
            \textbf{10} & \textbf{39.10/16.98/35.84} & 38.26/16.34/34.76 &  38.55/16.56/34.97 \\

             \textbf{10-aug} & 39.39/16.92/36.00 & 39.12/16.90/35.44 & \textbf{39.78/17.11/36.38} \\
              \textbf{10-cons} & \textbf{39.16/16.96/35.92} & 38.99/16.83/35.43 &  38.98/16.68/35.41 \\
             \Xhline{2\arrayrulewidth}
             \textbf{100} &  \textbf{40.55/18.01/37.03} & 40.13/17.88/36.67 & 40.14/17.88/36.62 \\
            %  \Xhline{2\arrayrulewidth}
             \textbf{100-aug} & \textbf{42.08/18.93/38.83} & 40.94/18.52/37.00 & 40.47/18.18/37.07  \\
            %  \Xhline{2\arrayrulewidth}
             \textbf{100-cons} & 41.12/18.34/37.51  & 40.84/18.09/37.28 & 
             \textbf{41.36/18.59/37.77} \\
             \Xhline{2\arrayrulewidth}
            % XSUM  
             \multicolumn{4}{c}{}   \\
            \Xhline{2\arrayrulewidth} 
            \textbf{Target Dataset} &   \multicolumn{3}{c}{XSum} \\
            \Xhline{2\arrayrulewidth}
            \textbf{Transfer from} & WikiTransfer & Reddit & BART \\
            \Xhline{2\arrayrulewidth}
            \textbf{0} & \textbf{31.85/10.44/23.75} & 24.04/6.43/18.99 & 19.87/2.75/15.66 \\
            \Xhline{2\arrayrulewidth}
            \textbf{10} & \textbf{34.95/12.61/26.58} & 30.69/10.22/23.29 & 22.45/5.94/17.23  \\
            % \Xhline{2\arrayrulewidth}
            \textbf{10-aug} & \textbf{34.98/12.73/26.79} & 31.03/10.23/23.29 & 26.10/8.19/20.18 \\
            % \Xhline{2\arrayrulewidth}
             \textbf{10-cons}  & \textbf{35.17/12.76/26.80} & 31.25/10.54/23.73  & 28.28/9.13/21.61 \\
            \Xhline{2\arrayrulewidth}
             \textbf{100} & \textbf{36.92/14.09/28.44} & 34.17/12.64/26.37 & 35.17/13.29/27.20  \\
            % \Xhline{2\arrayrulewidth}
             \textbf{100-aug} & \textbf{36.87/14.18/28.62} & 31.75/11.12/24.49 & 28.85/9.46/22.28 \\
            % \Xhline{2\arrayrulewidth}
            \textbf{100-cons} & \textbf{37.26/14.20/28.85} & 36.14/13.65/27.97 & 36.65/14.05/28.57 \\
            \Xhline{2\arrayrulewidth}
            %  Reddit
            \multicolumn{4}{c}{}   \\
            \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{3}{c}{Reddit} \\
            \Xhline{2\arrayrulewidth}
            \textbf{Transfer from} & WikiTransfer & CNNDM & BART \\
            \Xhline{2\arrayrulewidth}
            \textbf{0}  & \textbf{21.47}/4.10/17.62 & 21.37/\textbf{4.14/17.76} & 18.66/2.90/15.33 \\
            \Xhline{2\arrayrulewidth}
            \textbf{10}  & \textbf{27.88/7.62/22.09} & 26.55/6.83/21.29 & 19.37/3.51/15.72 \\
            % \Xhline{2\arrayrulewidth}
            \textbf{10-aug} & \textbf{28.07/7.70/22.47} & 26.88/6.95/21.46 & 21.39/4.57/17.22 \\
            % \Xhline{2\arrayrulewidth}
             \textbf{10-cons} & \textbf{28.42/7.88/22.32} & 27.20/7.14/21.67 & 20.42/3.97/16.45 \\
            \Xhline{2\arrayrulewidth}
              \textbf{100}  & \textbf{29.87/8.93/23.31} & 28.90/8.42/22.56 & 29.66/8.88/23.12 \\
            % \Xhline{2\arrayrulewidth}
             \textbf{100-aug} & \textbf{30.54/9.24/24.31} & 29.28/8.51/23.28 & 28.96/8.39/22.80  \\
            % \Xhline{2\arrayrulewidth}
             \textbf{100-cons} & 30.56/9.22/\textbf{24.38} & \textbf{30.78/9.45}/24.14 &\textbf{30.78}/9.22/23.32   \\
            \Xhline{2\arrayrulewidth}
            % BigPatent
             \multicolumn{4}{c}{}   \\
            \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{3}{c}{BigPatent} \\
            \Xhline{2\arrayrulewidth}
           \textbf{Transfer from} & WikiTransfer & CNNDM & BART \\
           \Xhline{2\arrayrulewidth}
          \textbf{0}   &  \textbf{35.58/10.91/31.53} & 33.57/9.34/25.76 & 32.56/9.64/29.27 \\
          \Xhline{2\arrayrulewidth}
              \textbf{10}  & \textbf{37.06/11.58/32.37} & 35.76/10.62/30.63 & 34.48/10.76/30.56 \\  
            %   \Xhline{2\arrayrulewidth}
              \textbf{10-aug} & \textbf{37.73/12.40/32.89} & 36.83/11.33/30.95 &  36.11/11.40/32.04 \\  
            %   \Xhline{2\arrayrulewidth}
              \textbf{10-cons}  & \textbf{37.64/12.24/33.05} &  36.11/10.84/30.64  & 33.99/10.48/30.45 \\  \Xhline{2\arrayrulewidth}
              \textbf{100}  & \textbf{39.61/13.53/}33.86 & 39.35/13.03/\textbf{33.88} & 39.06/13.04/33.61 \\ 
              
            %   \Xhline{2\arrayrulewidth}
                \textbf{100-aug}  & \textbf{40.95/14.05/35.03} & 38.88/12.69/32.88 & 38.77/12.88/33.55 \\  
                % \Xhline{2\arrayrulewidth} 
                \textbf{100-cons} & \textbf{39.87/13.76}/34.32 & 39.74/13.45/\textbf{34.49} & 39.46/13.37/34.28 \\  \Xhline{2\arrayrulewidth}
             
\end{tabular}}
\caption{A comparison of transfer results across datasets, training dataset size, data augmentation techniques, showing the generalizable and robust performance of our models transferred from WikiTransfer.}
\label{tab:table_all}
\end{table}
}

\newcommand{\TableComparePegasus}{
\begin{table*}[ht!]
\centering
\resizebox{2\columnwidth}{!}{\begin{tabular}{c | c c c | c c c} \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{3}{c|}{WikiTransfer} &  \multicolumn{3}{c}{Pegasus \cite{zhang2019pegasus}}  \\
          \Xhline{2\arrayrulewidth} 
          \# training samples   &  0 & 10 & 100 & 0 & 10  & 100 \\
          \Xhline{2\arrayrulewidth} 
          CNNDM   &  \textbf{39.11/17.25/35.73} & \textbf{39.39/16.92/36.00} & \textbf{42.08/18.93/38.83} & 32.90/13.28/29.38 & 37.25/15.84/33.49  & 40.28/18.21/37.03 \\
        %   \Xhline{2\arrayrulewidth} 
          XSum   &  \textbf{31.85/10.44/23.75} & \textbf{35.17/12.76/26.80} & 37.26/14.20/28.85 & 19.27/3.00/12.72 & 19.39/3.45/14.02/ & \textbf{39.07/16.44/31.27} \\
        %   \Xhline{2\arrayrulewidth} 
          Reddit   &  \textbf{21.47/4.10/17.62} & \textbf{28.42/7.88/22.32} & \textbf{30.56/9.22/24.38} & 14.66/3.06/10.17 & 15.36/2.91/10.76  & 16.64/4.09/12.92 \\
        %   \Xhline{2\arrayrulewidth} 
          BigPatent   &  \textbf{35.58/10.91/31.53} & \textbf{37.73/12.40/32.89} & \textbf{40.95/14.05/35.03} & 25.61/6.56/17.42 & 28.87/8.30/19.71  & 33.52/10.82/22.87 \\
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{A comparison of zero and few-shot performance between our best-performing WikiTransfer model (-aug in the case of CNNDM and BigPatent and -cons for XSum and Reddit) and the zero and few-shot results reported in \citet{zhang2019pegasus}.}
\label{tab:table_compare_pegasus}
\end{table*}
}


\newcommand{\TableHumanEvaluation}{
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{c | c c |  c c} \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{2}{c|}{CNNDM} &  \multicolumn{2}{c}{XSum}  \\
              &  Relevance & Consistency & Relevance & Consistency \\
          \Xhline{2\arrayrulewidth} 
          0   &  \textbf{4.37} & \textbf{4.71} &  3.75* &  \textbf{3.75} \\
          10-aug   &  4.31 & 4.76 &  3.77* & 4.10 \\
          100-aug   &  4.25 & 4.86 & \textbf{4.00}  &  4.04 \\
          Full supervision   &   4.31 & 4.86 &  4.11  & 3.98 \\
            \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{Summary relevance and factual consistency across CNNDM and XSum datasets with varying amounts of training data. All results except those with an asterisks do not differ in a statistically significant way (p-value of 0.05) from the full supervision score. Bold results emphasize the least amount of data to achieve statistically indistinguishable results from the fully-supervised results.}
\label{tab:table_human_evaluation}
\end{table}
}

\newcommand{\ExampleSummaries}{
\begin{table}[t!]
\centering
\small
\begin{tabularx}{\columnwidth}{|X|}
\hline
%  \\ \hline
\textbf{Source Document:} \textcolor{blue}{Ms Jones} told BBC Radio Wales she did not want to give up being an AM to go to Brussels to replace Nathan Gill, UKIP Wales leader. Mr Gill has been told by the UKIP assembly group and the UKIP party chairman Steve Crowther to stop "double-jobbing" as an AM and MEP. Mr Gill said those making such calls were doing it out of "malice". "We've got Brexit now and I think that, possibly, it may be best to leave that role unfilled," Ms Jones told the Good Morning Wales programme. "I'm surprised I've not been formally asked what I'd like to do." Ms Jones, the South Wales West AM, is one of two people who could take up the role of UKIP Wales MEP if Mr Gill made it vacant - the other being South Wales East AM David Rowlands...
% 
 \\ \hline \hline
% \\ \hline
% \hline

\textbf{0:} \textcolor{red}{Lorraine} Jones is a Welsh Labour Party Member of the Welsh Assembly for South Wales West.
 \\ \hline
\textbf{10-aug:} \textcolor{red}{Lorraine} Jones is a Welsh Labour member of the Welsh Assembly for South Wales West.
 \\ \hline
\textbf{100-aug:} Wales Assembly Member for South Wales West \textcolor{red}{Rachel} Jones says she has not been formally asked to become a UKIP MEP.
 \\ \hline
\textbf{Full supervision:} First Minister \textcolor{red}{Carwyn} Jones has said she is "surprised" she has not been asked to become a UKIP MEP.
 \\ \hline
 \textbf{Gold Summary:} UKIP's Welsh MEP post may be better left unfilled as a result of Brexit , party AM \textcolor{red}{Caroline} Jones has said .
  \\ \hline
\end{tabularx}
\caption{An example of WikiTransfer model output across dataset size used in fine-tuning, illustrating how model output style and hallucinated entities differ as the model moves from Wikipedia pretraining as a source of knowledge to the target dataset. Text not stated in the source document is highlighted in red.}
\label{tab:example_summaries}
\end{table}
}
% She would, in theory, have first refusal over Mr Rowlands as she was third in the 2014 UKIP European Parliament election list and Mr Rowlands was fourth. The number two candidate, James Cole, is no longer in the party. Asked if she would give up her position as AM to become an MEP, she said: "No I wouldn't. I'm not interested. Since becoming an AM I've thrown myself totally into what I'm elected to do. "They'd have to ask David Rowlands obviously but neither of us have formally been asked, although David may say 'oh no I'm settling in in his role', and he is actually, he's doing very well. "Quite frankly I think it's impossible to do two jobs, especially when one is in Brussels and Strasbourg and the other is in the Welsh Assembly. It's a very difficult situation."
% Media playback is unsupported on your device 15 March 2015 Last updated at 14:00 GMT President Baldwin Lonsdale said Cyclone Pam had destroyed most buildings in the capital Port Vila. 267,000 people live in Vanuatu, spread over 65 small islands. The cyclone did not follow the course it was expected to take, and hit populated areas. It has destroyed schools and medical clinics, and thousands of homes.





\newcommand{\TableAllUda}{
\begin{table}[t!]
\tiny
\centering
\resizebox{\columnwidth}{!}{\begin{tabular}{ c c c c } \Xhline{2\arrayrulewidth}
            % CNNDM
             \textbf{Target Dataset} &  \multicolumn{3}{c}{CNNDM}  \\
             \Xhline{2\arrayrulewidth}
             \textbf{Transfer from} & WikiTransfer & Reddit & BART \\ \Xhline{2\arrayrulewidth}
            % \textbf{0} & \textbf{39.11/17.25/35.73} & 36.81/14.18/32.62 & 35.98/15.1/32.97  \\  \Xhline{2\arrayrulewidth}
            % \textbf{10} & \textbf{39.10/16.98/35.84} & 38.26/16.34/34.76 &  38.55/16.56/34.97 \\ \Xhline{2\arrayrulewidth}
            %  \textbf{10-aug} & 39.39/16.92/36.00 & 39.12/16.9/35.44 & \textbf{39.78/17.11/36.38} \\
            %  \Xhline{2\arrayrulewidth}
              \textbf{10-UDA} & \textbf{39.51/17.2/35.93 } &  38.86/16.83/35.26  &  37.81/16.82/34.64 \\
            %  \Xhline{2\arrayrulewidth}
            %  \textbf{100} &  \textbf{40.55/18.01/37.03} & 40.13/17.88/36.67 & 40.14/17.88/36.62 \\
            %  \Xhline{2\arrayrulewidth}
            %  \textbf{100-aug} & \textbf{42.08/18.93/38.83} & 40.94/18.52/37.00 & 40.47/18.18/37.07  \\
             \Xhline{2\arrayrulewidth}
             \textbf{100-UDA} & 39.89/17.27/36.26  & \textbf{40.19/17.91/36.98} & 38.43/17.22/35.49  \\
             \Xhline{2\arrayrulewidth}
            % XSUM  
             \multicolumn{4}{c}{}   \\
            \Xhline{2\arrayrulewidth} 
            \textbf{Target Dataset} &   \multicolumn{3}{c}{XSum} \\
            \Xhline{2\arrayrulewidth}
            \textbf{Transfer from} & WikiTransfer & Reddit & BART \\
            \Xhline{2\arrayrulewidth}
            % \textbf{0} & \textbf{31.85/10.44/23.75} & 24.04/6.43/18.99 & 20.26/31.87/5.68 \\
            % \Xhline{2\arrayrulewidth}
            % \textbf{10} & \textbf{34.95/12.61/26.58} & 30.69/10.22/23.29 & 22.45/5.94/17.23  \\ \Xhline{2\arrayrulewidth}
            % \textbf{10-aug} & \textbf{34.98/12.73/26.79}  & 31.03/10.23/23.29 & 26.10/8.19/20.18 \\
            % \Xhline{2\arrayrulewidth}
             \textbf{10-UDA}  & \textbf{35.09/12.86/26.94} & 29.34/9.56/22.6   & 19.75/3.19/15.09  \\
            \Xhline{2\arrayrulewidth}
            %  \textbf{100} & \textbf{36.92/14.09/28.44} & 34.17/12.64/26.37 & 35.17/13.29/27.20  \\
            % \Xhline{2\arrayrulewidth}
            %  \textbf{100-aug} & \textbf{36.87/14.18/28.62} & 31.75/11.12/24.49 & 28.85/9.46/22.28 \\
            % \Xhline{2\arrayrulewidth}
            \textbf{100-UDA} & \textbf{36.57/13.89/28.42} & 33.91/12.23/26.05  & 26.44/7.97/20.35   \\
            \Xhline{2\arrayrulewidth}
            %  Reddit
            \multicolumn{4}{c}{}   \\
            \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{3}{c}{Reddit} \\
            \Xhline{2\arrayrulewidth}
            \textbf{Transfer from} & WikiTransfer & CNNDM & BART \\
            \Xhline{2\arrayrulewidth}
            % \textbf{0}  & \textbf{21.47}/4.10/17.62 & 21.37/\textbf{4.14/17.76} & 18.66/2.90/15.33 \\
            % \Xhline{2\arrayrulewidth}
            % \textbf{10}  & \textbf{27.88/7.62/22.09} & 26.55/6.83/21.29 & 19.37/3.51/15.72 \\
            % \Xhline{2\arrayrulewidth}
            % \textbf{10-aug} & \textbf{28.07/7.70/22.47} & 26.88/6.95/21.46 & 21.39/4.57/17.22 \\
            % \Xhline{2\arrayrulewidth}
             \textbf{10-UDA} & \textbf{27.6/7.19/22.37} & 25.21/5.96/20.63  &  20.9/4.16/16.82  \\
            \Xhline{2\arrayrulewidth}
            %   \textbf{100}  & \textbf{29.87/8.93/23.31} & 28.90/8.42/22.56 & 29.66/8.88/23.12 \\
            % \Xhline{2\arrayrulewidth}
            %  \textbf{100-aug} & \textbf{30.54/9.24/24.31} & 29.28/8.51/23.28 & 28.96/8.39/22.80  \\
            % \Xhline{2\arrayrulewidth}
             \textbf{100-UDA} & \textbf{29.91/8.35/23.93 } & 28.28/7.68/22.83  & 27.67/7.46/21.81   \\
            \Xhline{2\arrayrulewidth}
            % BigPatent
             \multicolumn{4}{c}{}   \\
            \Xhline{2\arrayrulewidth}
            \textbf{Target Dataset} &  \multicolumn{3}{c}{BigPatent} \\
            \Xhline{2\arrayrulewidth}
           \textbf{Transfer from} & WikiTransfer & CNNDM & BART \\
           \Xhline{2\arrayrulewidth}
        %   \textbf{0}   &  \textbf{35.58/10.91/31.53} & 33.57/9.34/25.76 & 32.56/9.64/29.27 \\
        %   \Xhline{2\arrayrulewidth}
        %       \textbf{10}  & \textbf{37.06/11.58/32.37} & 35.76/10.62/30.63 & 34.48/10.76/30.56 \\  \Xhline{2\arrayrulewidth}
            %   \textbf{10-aug} & \textbf{37.73/12.40/32.89} & 36.83/11.33/30.95 &  36.11/11.40/32.04 \\  \Xhline{2\arrayrulewidth}
              \textbf{10-UDA}  & \textbf{36.58/11.45/32.29} &  33.77/9.45/29.19   & 32.32/10.0/28.98  \\  \Xhline{2\arrayrulewidth}
            %   \textbf{100}  & \textbf{39.61/13.53/}33.86 & 39.35/13.03/\textbf{33.88} & 39.06/13.04/33.61 \\  \Xhline{2\arrayrulewidth}
            %     \textbf{100-aug}  & \textbf{40.95/14.05/35.03} & 38.88/12.69/32.88 & 38.77/12.88/33.55 \\  \Xhline{2\arrayrulewidth} 
                \textbf{100-UDA} & \textbf{40.25/13.77/35.09 }  &  39.04/12.99/34.41  & 38.2/12.7/34.16 5 \\  \Xhline{2\arrayrulewidth}
             
\end{tabular}}
\caption{Results from experiments using the original formulation of UDA \citet{xie2019unsupervised} on 10 examples.}
\label{tab:table_all_uda}
\end{table}
}

% need to update with the latest numbers
\newcommand{\FigureResultsAllBold}{
\begin{figure}[t]
    \centering
    \includegraphics[width=.5\textwidth,height=.5\textheight,keepaspectratio]{plots/results_all_bold_nolegend.pdf}
    \caption{\textcolor{black}{ROUGE-1}/\textcolor{red}{2}/\textcolor{blue}{L} scores across datasets, training dataset size, data augmentation (\textbf{*-a}), and consistency loss (\textbf{*-c}) showing the generalizable and robust performance of models transferred from WikiTransfer. }
    \label{fig:results_all_plot}
\end{figure} 
}

==> misc.tex <==

% \newcommand{\ZeroShotAllDatasets}{
% \begin{table}[t!]
% \centering
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c  c} \Xhline{2\arrayrulewidth}
%              \textbf{Target Dataset} & \textbf{SOTA Full Dataset} & \textbf{WikiTransfer} & \textbf{Best Transfer} \\ \Xhline{\arrayrulewidth}
%               CNNDM & 45.94 \small{\cite{dou2020gsum}} & 39.11 & 36.81 (from Reddit)   \\
%               XSum & 47.21 \small{\cite{zhang2019pegasus}} & 31.85 & 24.04 (from Reddit)   \\ 
%              Reddit & 32.76 (ours) & 21.47 & 21.37 (from CNNDM)   \\
%              BigPatent & 53.63 \small{\cite{zhang2019pegasus}} & 35.58 & 33.57 (from CNNDM)   \\
             
%              \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Comparison of ROUGE-1 zero-shot transfer performance from dataset-specific WikiTransfer vs. transfer from another dataset. The dataset from which zero-shot transfer performed the best is shown in parentheses.}
% %  State-of-the-art supervised performance on that dataset are shown for comparison.
% \label{tab:zero_shot}
% \end{table}
% }

% \newcommand{\ZeroShotAllDatasets}{
% \begin{table}[t!]
% \centering
% \resizebox{\columnwidth}{!}{\begin{tabular}{c c c  c} \Xhline{2\arrayrulewidth}
%              \textbf{Target Dataset} & \textbf{SOTA Full Dataset} & \textbf{WikiTransfer} & \textbf{Transfer (Best)} \\ \Xhline{\arrayrulewidth}
%               CNNDM & 45.94 \tiny{\cite{dou2020gsum}} (44.16) & 39.11 & 36.81 (from Reddit)   \\
%               XSum & 47.21 (45.14) & 31.85 & 24.04 (from Reddit)   \\ 
%              Reddit & 32.76 & 21.47 & 21.37 (from CNNDM)   \\
%              BigPatent & 53.63 (43.34) & 35.58 & 33.57 (from CNNDM)   \\
             
%              \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Comparison of ROUGE-1 zero-shot transfer performance from dataset-specific WikiTransfer vs. transfer from another dataset. The best-performing zero-shot model is shown the right column in parentheses. We show the state-of-the-art supervised performance on that dataset and in parentheses the performance of our BART model trained on that dataset. }
% \label{tab:zero_shot}
% \end{table}
% }



% \newcommand{\TableAllUda}{
% \begin{table}[t!]
% \tiny
% \centering
% \resizebox{\columnwidth}{!}{\begin{tabular}{ c c c c } \Xhline{2\arrayrulewidth}
%             % CNNDM
%              \textbf{Target Dataset} &  \multicolumn{3}{c}{CNNDM}  \\
%              \Xhline{2\arrayrulewidth}
%              \textbf{Transfer from} & WikiTransfer & Reddit & BART \\ \Xhline{2\arrayrulewidth}
%             % \textbf{0} & \textbf{39.11/17.25/35.73} & 36.81/14.18/32.62 & 35.98/15.1/32.97  \\  \Xhline{2\arrayrulewidth}
%             % \textbf{10} & \textbf{39.10/16.98/35.84} & 38.26/16.34/34.76 &  38.55/16.56/34.97 \\ \Xhline{2\arrayrulewidth}
%             %  \textbf{10-aug} & 39.39/16.92/36.00 & 39.12/16.9/35.44 & \textbf{39.78/17.11/36.38} \\
%             %  \Xhline{2\arrayrulewidth}
%               \textbf{10-UDA} & \textbf{39.51/17.2/35.93 } &  38.86/16.83/35.26  &  37.81/16.82/34.64 \\
%             %  \Xhline{2\arrayrulewidth}
%             %  \textbf{100} &  \textbf{40.55/18.01/37.03} & 40.13/17.88/36.67 & 40.14/17.88/36.62 \\
%             %  \Xhline{2\arrayrulewidth}
%             %  \textbf{100-aug} & \textbf{42.08/18.93/38.83} & 40.94/18.52/37.00 & 40.47/18.18/37.07  \\
%              \Xhline{2\arrayrulewidth}
%             %  \textbf{100-UDA} & 39.89/17.27/36.26  & \textbf{40.19/17.91/36.98} & 38.43/17.22/35.49  \\
%             %  \Xhline{2\arrayrulewidth}
%             % XSUM  
%              \multicolumn{4}{c}{}   \\
%             \Xhline{2\arrayrulewidth} 
%             \textbf{Target Dataset} &   \multicolumn{3}{c}{XSum} \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Transfer from} & WikiTransfer & Reddit & BART \\
%             \Xhline{2\arrayrulewidth}
%             % \textbf{0} & \textbf{31.85/10.44/23.75} & 24.04/6.43/18.99 & 20.26/31.87/5.68 \\
%             % \Xhline{2\arrayrulewidth}
%             % \textbf{10} & \textbf{34.95/12.61/26.58} & 30.69/10.22/23.29 & 22.45/5.94/17.23  \\ \Xhline{2\arrayrulewidth}
%             % \textbf{10-aug} & \textbf{34.98/12.73/26.79} & 31.03/10.23/23.29 & 26.10/8.19/20.18 \\
%             % \Xhline{2\arrayrulewidth}
%              \textbf{10-UDA}  & \textbf{35.09/12.86/26.94} & 29.34/9.56/22.6   & 19.75/3.19/15.09  \\
%             \Xhline{2\arrayrulewidth}
%             %  \textbf{100} & \textbf{36.92/14.09/28.44} & 34.17/12.64/26.37 & 35.17/13.29/27.20  \\
%             % \Xhline{2\arrayrulewidth}
%             %  \textbf{100-aug} & \textbf{36.87/14.18/28.62} & 31.75/11.12/24.49 & 28.85/9.46/22.28 \\
%             % \Xhline{2\arrayrulewidth}
%             % \textbf{100-UDA} & \textbf{36.57/13.89/28.42} & 33.91/12.23/26.05  & 26.44/7.97/20.35   \\
%             % \Xhline{2\arrayrulewidth}
%             %  Reddit
%             \multicolumn{4}{c}{}   \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Target Dataset} &  \multicolumn{3}{c}{Reddit} \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Transfer from} & WikiTransfer & CNNDM & BART \\
%             \Xhline{2\arrayrulewidth}
%             % \textbf{0}  & \textbf{21.47}/4.10/17.62 & 21.37/\textbf{4.14/17.76} & 18.66/2.90/15.33 \\
%             % \Xhline{2\arrayrulewidth}
%             % \textbf{10}  & \textbf{27.88/7.62/22.09} & 26.55/6.83/21.29 & 19.37/3.51/15.72 \\
%             % \Xhline{2\arrayrulewidth}
%             % \textbf{10-aug} & \textbf{28.07/7.70/22.47} & 26.88/6.95/21.46 & 21.39/4.57/17.22 \\
%             % \Xhline{2\arrayrulewidth}
%              \textbf{10-UDA} & \textbf{27.6/7.19/22.37} & 25.21/5.96/20.63  &  20.9/4.16/16.82  \\
%             \Xhline{2\arrayrulewidth}
%             %   \textbf{100}  & \textbf{29.87/8.93/23.31} & 28.90/8.42/22.56 & 29.66/8.88/23.12 \\
%             % \Xhline{2\arrayrulewidth}
%             %  \textbf{100-aug} & \textbf{30.54/9.24/24.31} & 29.28/8.51/23.28 & 28.96/8.39/22.80  \\
%             % \Xhline{2\arrayrulewidth}
%             %  \textbf{100-UDA} & \textbf{29.91/8.35/23.93 } & 28.28/7.68/22.83  & 27.67/7.46/21.81   \\
%             % \Xhline{2\arrayrulewidth}
%             % BigPatent
%              \multicolumn{4}{c}{}   \\
%             \Xhline{2\arrayrulewidth}
%             \textbf{Target Dataset} &  \multicolumn{3}{c}{BigPatent} \\
%             \Xhline{2\arrayrulewidth}
%           \textbf{Transfer from} & WikiTransfer & CNNDM & BART \\
%           \Xhline{2\arrayrulewidth}
%         %   \textbf{0}   &  \textbf{35.58/10.91/31.53} & 33.57/9.34/25.76 & 32.56/9.64/29.27 \\
%         %   \Xhline{2\arrayrulewidth}
%         %       \textbf{10}  & \textbf{37.06/11.58/32.37} & 35.76/10.62/30.63 & 34.48/10.76/30.56 \\  \Xhline{2\arrayrulewidth}
%             %   \textbf{10-aug} & \textbf{37.73/12.40/32.89} & 36.83/11.33/30.95 &  36.11/11.40/32.04 \\  \Xhline{2\arrayrulewidth}
%               \textbf{10-UDA}  & \textbf{36.58/11.45/32.29} &  33.77/9.45/29.19   & 32.32/10.0/28.98  \\  \Xhline{2\arrayrulewidth}
%             %   \textbf{100}  & \textbf{39.61/13.53/}33.86 & 39.35/13.03/\textbf{33.88} & 39.06/13.04/33.61 \\  \Xhline{2\arrayrulewidth}
%             %     \textbf{100-aug}  & \textbf{40.95/14.05/35.03} & 38.88/12.69/32.88 & 38.77/12.88/33.55 \\  \Xhline{2\arrayrulewidth} 
%                 % \textbf{100-UDA} & \textbf{40.25/13.77/35.09 }  &  39.04/12.99/34.41  & 38.2/12.7/34.16 5 \\  \Xhline{2\arrayrulewidth}
             
% \end{tabular}}
% \caption{Results from experiments using the original formulation of UDA \citet{xie2019unsupervised} on 10 examples.}
% \label{tab:table_all_uda}
% \end{table}
% }
